Analogical Reasoning Within a Conceptual Hyperspace

We propose an approach to analogical inference that marries the neuro-symbolic computational power of complex-sampled hyperdimensional computing (HDC) with Conceptual Spaces Theory (CST), a promising theory of semantic meaning. CST sketches, at an abstract level, approaches to analogical inference that go beyond the standard predicate-based structure mapping theories. But it does not describe how such an approach can be operationalized. We propose a concrete HDC-based architecture that computes several types of analogy classified by CST. We present preliminary proof-of-concept experimental results within a toy domain and describe how it can perform category-based and property-based analogical reasoning.

==> algorithm.tex <==
\begin{algorithm}
    \caption{map}
    \begin{algorithmic}[1] %[1] enables line numbers
    \STATE Input: 
    \STATE Output:
    \end{algorithmic}
\end{algorithm}


